Machine Translation between Vietnamese and English: an Empirical Study

Machine translation is shifting to an end-to-end approach based on deep neural networks. The state of the art achieves impressive results for popular language pairs such as English - French or English - Chinese. However for English - Vietnamese the shortage of parallel corpora and expensive hyper-parameter search present practical challenges to neural-based approaches. This paper highlights our efforts on improving English-Vietnamese translations in two directions: (1) Building the largest open Vietnamese - English corpus to date, and (2) Extensive experiments with the latest neural models to achieve the highest BLEU scores. Our experiments provide practical examples of effectively employing different neural machine translation models with low-resource language pairs.

==> dih.tex <==
%auto-ignore
% Cac macro dau tieng Viet
\catcode`\@=11
\def\dd{\leavevmode\setbox0\hbox{d}\dimen@\wd0%
\rlap{\kern.3333\dimen@\raise1.2ex\vbox{\hrule width.5\dimen@}}d}

\def\DD{\leavevmode\setbox0\hbox{D}\dimen@\wd0%
\rlap{\kern.05\dimen@\raise0.8ex\vbox{\hrule width.5\dimen@}}D}

%\def\dd{d\kern-.46em\char '26}
%\def\DD{D\kern-.7em\raise0.4ex\hbox{\char '55}\kern.33em}
\def\is{\' \i }
\def\ih{\` \i }
\def\ihoi{\i \kern-.270em\raise.16ex\hbox{\char'47}\kern-.01em}
\def\inga{\~ \i }
\def\ing{\d i}
\def\ys{\' y}
\def\yh{\` y}
\def\yhoi{y\kern-.370em\raise.16ex\hbox{\char'47}\kern.1em}
\def\yn{\~ y}
\def\yng{\d y}
\def\as{\' a}
\def\ah{\` a}
\def\ahoi{a\kern-.370em\raise.16ex\hbox{\char'47}\kern.1em}
\def\an{\~ a}
\def\ang{\d a}
\def\us{\' u}
\def\uh{\` u}
\def\uhoi{u\kern-.370em\raise.16ex\hbox{\char'47}\kern.1em}
\def\un{\~ u}
\def\ung{\d u}
\def\es{\' e}
\def\eh{\` e}
\def\ehoi{e\kern-.370em\raise.16ex\hbox{\char'47}\kern.1em}
\def\en{\~ e}
\def\eng{\d e}
\def\os{\' o}
\def\oh{\` o}
\def\ohoi{o\kern-.370em\raise.16ex\hbox{\char'47}\kern.1em}
\def\on{\~ o}
\def\ong{\d o}
\def\oo{\^ o}
\def\oos{{\accent"5E o}\kern-.385em\raise.2ex
           \hbox{\char'23 }\kern-.1em}
\def\ooh{{\accent"5E o}\kern-.36em\raise.3ex
           \hbox{\char'22}\kern-.1em}
\def\oohoi{{\accent"5E o}\kern-.21em\raise.35ex
           \hbox{\char'47 }\kern-0.03em}
\def\oon{{\accent"5E o}\kern-.470em
           \raise.34ex\hbox{\char'176}}
\def\oong{\d {\accent"5E o}}
\def\aa{\^ a}
\def\aas{{\accent"5E a}\kern-.385em
       \raise.2ex\hbox{\char'23}\kern-.08em}
\def\aah{{\accent"5E a}\kern-.62em
       \raise.2ex\hbox{\char'22}\kern.12em}
\def\aahoi{{\accent"5E a}\kern-.21em
       \raise.35ex\hbox{\char'47 }\kern-.03em}
\def\aan{{\accent"5E a}\kern-.470em
       \raise.3ex\hbox{\char'176}}
\def\aang{\d {\accent"5E a}}
\def\ee{\^ e}
\def\ees{{\accent"5E e}\kern-.385em
       \raise.2ex\hbox{\char'23}\kern-.08em}
\def\eeh{{\accent"5E e}\kern-.62em
       \raise.2ex\hbox{\char'22}\kern.14em}
\def\eehoi{{\accent"5E e}\kern-.21em
       \raise.35ex\hbox{\char'47 }\kern-.01em}
\def\een{{\accent"5E e}\kern-.470em
       \raise.3ex\hbox{\char'176}}
\def\eeng{\d {\accent"5E e}}
\def\aw{\u a}
\def\aws{{\accent"15 a}\kern-.470em
       \raise.3ex\hbox{\char'23}\kern-.002em}
\def\awh{{\accent"15 a}\kern-.50em
       \raise.3ex\hbox{\char'22}\kern.05em}
\def\awhoi{{\accent"15 a}\kern-.410em
       \raise.3ex\hbox{\char'47}\kern.16em}
\def\awn{{\accent"15 a}\kern-.470em
       \raise.45ex\hbox{\char'176}}
\def\awng{\d {\accent"15 a}}
\def\uw{u\kern-.44em\raise.82ex\hbox{
       \vrule width .12em height .0ex depth .075ex 
       \kern-0.16em \char'56}\kern-.07em}
\def\uws{\' \uw }
\def\uwh{\` \uw }
\def\uwhoi{\uw \kern-.450em\raise.16ex
       \hbox{\char'47}\kern.175em}
\def\uwn{\~ \uw }
\def\uwng{\d \uw }
\def\ow{o\kern-.42em\raise.82ex\hbox{
       \vrule width .12em height .0ex depth .075ex 
       \kern-0.16em \char'56}\kern-.07em}
\def\ows{\' \ow }
\def\owh{\` \ow }
\def\owhoi{\ow \kern-.450em\raise.16ex
       \hbox{\char'47}\kern.175em}
\def\own{\~ \ow }
\def\owng{\d \ow }
\def\IS{\' I}
\def\IH{\` I}
\def\IHOI{I \kern-.63em\raise.80ex
       \hbox{\char'47}\kern.018em}
\def\INGA{\~ I}
\def\ING{\d I}
\def\YS{\' Y}
\def\YH{\` Y}
\def\YHOI{Y\kern-.46em\raise.80ex
       \hbox{\char'47}\kern.18em}
\def\YN{\~ Y}
\def\YNG{\d Y}
\def\AS{\' A}
\def\AH{\` A}
\def\AHOI{A\kern-.46em\raise.80ex\hbox{\char'47}\kern.18em}
\def\AN{\~ A}
\def\ANG{\d A}
\def\US{\' U}
\def\UH{\` U}
\def\UHOI{U\kern-.46em\raise.80ex\hbox{\char'47}\kern.18em}
\def\UN{\~ U}
\def\UNG{\d U}
\def\ES{\' E}
\def\EH{\` E}
\def\EHOI{E\kern-.46em\raise.80ex\hbox{\char'47}\kern.18em}
\def\EN{\~ E}
\def\ENG{\d E}
\def\OS{\' O}
\def\OH{\` O}
\def\OHOI{O\kern-.46em\raise.80ex\hbox{\char'47}\kern.2em}
\def\ON{\~ O}
\def\ONG{\d O}
\def\OO{\^ O}
\def\OOS{{\accent"5E O}\kern-.5em
      \raise.8ex\hbox{\char'23 }}
\def\OOH{{\accent"5E O}\kern-.48em
      \raise.9ex\hbox{\char'22}\kern-.08em}
\def\OOHOI{{\accent"5E O}\kern-.33em
      \raise1.02ex\hbox{\char'47 }\kern.04em}
\def\OON{{\accent"5E O}\kern-.60em
      \raise.9ex\hbox{\char'176}\kern.1em}
\def\OONG{\d {\accent"5E O}}
\def\AA{\^ A}
\def\AAS{{\accent"5E A}\kern-.5em
      \raise.8ex\hbox{\char'23 }}
\def\AAH{{\accent"5E A}\kern-.78em
      \raise.8ex\hbox{\char'22}\kern.28em}
\def\AAHOI{{\accent"5E A}\kern-.33em
      \raise1.02ex\hbox{\char'47 }\kern.04em}
\def\AAN{{\accent"5E A}\kern-.60em
      \raise.9ex\hbox{\char'176}\kern.07em}
\def\AANG{\d {\accent"5E A}}
\def\EE{\^ E}
\def\EES{{\accent"5E E}\kern-.5em
      \raise.8ex\hbox{\char'23 }}
\def\EEH{{\accent"5E E}\kern-.78em
      \raise.8ex\hbox{\char'22}\kern.28em }
\def\EEHOI{{\accent"5E E}\kern-.33em
      \raise1.02ex\hbox{\char'47 }\kern.04em}
\def\EEN{{\accent"5E E}\kern-.60em
      \raise.9ex\hbox{\char'176}\kern.1em}
\def\EENG{\d {\accent"5E E}}
\def\AW{\u A}
\def\AWS{{\accent"15 A}\kern-.620em
      \raise.85ex\hbox{\char'23}\kern.05em}
\def\AWH{{\accent"15 A}\kern-.60em
      \raise.85ex\hbox{\char'22}\kern.05em}
\def\AWHOI{{\accent"15 A}\kern-.530em
      \raise.88ex\hbox{\char'47}\kern.18em}
\def\AWN{{\accent"15 A}\kern-.57em
      \raise.97ex\hbox{\char'176}\kern.05em}
\def\AWNG{\d {\accent"15 A}}
\def\UW{U\kern-.42em\raise1.36ex\hbox{
      \vrule width .13em height .0ex depth .075ex 
      \kern-0.16em \char'56}\kern-.07em}
\def\UWS{\' \UW }
\def\UWH{\` \UW }
\def\UWHOI{\UW \kern-.48em\raise.80ex\hbox{\char'47}\kern.21em}
\def\UWN{\~ \UW }
\def\UWNG{\d \UW }
\def\OW{O\kern-.460em\raise1.36ex\hbox{
      \vrule width .13em height .0ex depth .075ex 
      \kern-0.16em \char'56}\kern-.07em}
\def\OWS{\' \OW }
\def\OWH{\` \OW }
\def\OWHOI{\OW \kern-.540em\raise.80ex\hbox{\char'47}\kern.25em}
\def\OWN{\~ \OW }
\def\OWNG{\d \OW }
\catcode`\@=\active

